High-Fidelity Clothed Avatar Reconstruction from a Single Image

This paper presents a framework for efficient 3D clothed avatar reconstruction. By combining the advantages of the high accuracy of optimization-based methods and the efficiency of learning-based methods, we propose a coarse-to-fine way to realize a high-fidelity clothed avatar reconstruction (CAR) from a single image. At the first stage, we use an implicit model to learn the general shape in the canonical space of a person in a learning-based way, and at the second stage, we refine the surface detail by estimating the non-rigid deformation in the posed space in an optimization way. A hyper-network is utilized to generate a good initialization so that the convergence o f the optimization process is greatly accelerated. Extensive experiments on various datasets show that the proposed CAR successfully produces high-fidelity avatars for arbitrarily clothed humans in real scenes.

==> figures/body-refine.tex <==
\begin{figure}
    \centering
  %  \vspace{-1.0 em}
    \includegraphics[trim=000mm 000mm 000mm 000mm, clip=true, width=1.00\linewidth]{photos/normal-alignment.pdf}
    \vspace{-1.5em}
    \caption{\smpl refinement using a feedback loop.}
     \label{fig:normal-body-refinement}
    \vspace{-1.5 em}
\end{figure}



==> figures/datasize.tex <==
\begin{figure}
\centering
    \includegraphics[trim=004mm 006mm 005mm 008.7mm, clip=true, width=1.0 \linewidth]{photos/datasize.pdf}
    \caption{
                Reconstruction error \wrt training-data size. 
                ``Dataset size'' is defined as the ratio \wrt the $450$ scans used in \cite{saito2019pifu, saito2020pifuhd}. 
                The ``8x'' setting is all $3,709$ scans of \agora~\cite{patel2021agora} and \thuman~\cite{zheng2019deephuman}. 
    }
    \label{fig:datasize}
\end{figure}



==> figures/demo.tex <==
\begin{figure*}
\centering{
    \begin{subfigure}{\linewidth}
        \includegraphics[trim=000mm 000mm 000mm 000mm, clip=true, width=1.0\linewidth]{photos/demo.pdf}
        \caption{
                    \modelname reconstructions for in-the-wild images with extreme poses (\cref{sec: application ICON}).
        }
        \label{fig:demo}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{photos/scanimate.pdf}
	    \caption{
	                Avatar creation from images with \scanimate (\cref{sec: application SCANimate}).  
	                The input per-frame meshes are reconstructed with \modelname.
	    }
	    \label{fig:scanimate}
    \end{subfigure}}
    \caption{
                \modelname results for two applications (\cref{sec: applications}). 
                We show two views for each mesh, \ie, a front (\textcolor{frontcolor}{blue}) and a rotated (\textcolor{sidecolor}{bronze}) view.
    }
\end{figure*}



==> figures/failure-small.tex <==
\begin{figure}
\centerline{ 
\includegraphics[width=\linewidth]{photos/failure-small.pdf}}
    \vspace{-0.5 em}
    \caption{
                Failure cases of \modelname for extreme clothing, pose, or camera view.
                We show the front (\textcolor{frontcolor}{blue}) and rotated (\textcolor{sidecolor}{bronze}) views. 
    }
    \label{fig:failure small}
\end{figure}



==> figures/normal-pred.tex <==
\begin{figure}
    \centering
    \vspace{-0.5 em}
    \includegraphics[trim=003mm 000mm 000mm 003mm, clip=true, width=1.0\linewidth]{photos/normal-pred.pdf}
    \vspace{-1.7 em}
    \caption{Normal prediction ($\predCloNormImg$) w/ and w/o \smpl prior ($\bodyNormImgFB$).}
    \label{fig:normal-prior}
    \vspace{-0.5 em}
\end{figure}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> paper/05_applications.tex <==
\section{Applications}
\label{sec: applications}


\subsection{Reconstruction from in-the-wild images}
\label{sec: application ICON}


We collect $200$ in-the-wild images from Pinterest that show people performing parkour, sports, street dance, and kung fu. 
These images are unseen during training. 
We show qualitative results for \modelname in \cref{fig:demo} and comparisons to SOTA in \cref{fig:motivation}; for more results see our \video and \suppl 

To evaluate the perceived realism of our results, we compare \modelname to \pifuSIM, \pamirSIM, and the original \pifuhd~\cite{saito2020pifuhd} in a perceptual study. 
\modelname, \pifuSIM and \text{\pamirSIM} are trained on all $3,709$ scans of \agora~\cite{patel2021agora} and \thuman~\cite{zheng2019deephuman} (``8x'' setting in \cref{fig:datasize}). 
For \pifuhd we use its pre-trained model. 
In the study, participants were shown an image and either a rendered result of \modelname or of another method.
Participants were asked to choose the result that best represents the shape \change{of the} human in the image. 
We report the percentage of trails in which participants preferred the baseline methods over \modelname in \cref{tab: perceptual study}; \mbox{p-values} correspond to the null-hypothesis that two methods perform equally well. 
\change{For details on the study, example stimuli, catch trials, etc.~see \suppl} 


\subsection{Animatable avatar creation from video}
\label{sec: application SCANimate}


Given a sequence of images with the same subject in various poses, we create an animatable avatar with the help of \scanimate~\cite{saito2021scanimate}.
First, we use \modelname to reconstruct a \threeD clothed-human mesh per frame. 
Then,  we feed these meshes to \scanimate. 
\modelname's robustness to diverse poses enables us to learn a clothed avatar with pose-dependent clothing deformation.
Unlike raw \threeD scans, which are taken with multi-view systems, \modelname operates on a single image and its reconstructions are more reliable for observed body regions than for occluded ones. 
Thus, we reformulate the loss of \scanimate to downweight occluded regions \highlight{depending on camera viewpoint}. Results are shown in \cref{fig:teaser} and \cref{fig:scanimate}; for animations see the \video on our \href{https://icon.is.tue.mpg.de}{webpage}. 

\input{figures/failure-small}
\input{tabs/perceptual_study}
\input{figures/demo}



==> tabs/benchmark.tex <==
\begin{table*}
\centering{
\resizebox{1.0\linewidth}{!}{
  \begin{tabular}{c|l|c|ccc|ccc|ccc|aaa}
    & Methods & \smplx & \multicolumn{3}{c|}{\agora-50} & \multicolumn{3}{c|}{\cape-FP} & \multicolumn{3}{c|}{\cape-NFP} & \multicolumn{3}{a}{\cape}\\
    & & condition. & Chamfer $\downarrow$ & P2S $\downarrow$ & Normals $\downarrow$ & Chamfer $\downarrow$ & P2S $\downarrow$ & Normals $\downarrow$ & Chamfer $\downarrow$ & P2S $\downarrow$ & Normals $\downarrow$ & Chamfer $\downarrow$ & P2S $\downarrow$ & Normals $\downarrow$\\
    \shline
    Ours & $\text{\modelname}$ & \cmark  & 1.204 & 1.584 & 0.060 & 1.233 & \textbf{1.170} & 0.072 & 1.096 & \textbf{1.013} & 0.063 & \textbf{1.142} & \textbf{1.065} & 0.066\\
    \hline
    \multirow{6}{*}{A} 
    & \makebox[1.3cm][l]{$\text{\pifu}$}~\cite{saito2019pifu} &  \xmark & 3.453 & 3.660 & 0.094 & 2.823 & 2.796 & 0.100 & 4.029 & 4.195 & 0.124 & 3.627 & 3.729 & 0.116\\
    & \makebox[1.3cm][l]{$\text{\pifuhd}$}~\cite{saito2020pifuhd} &  \xmark & 3.119 & 3.333 & 0.085 & 2.302 & 2.335 & 0.090 & 3.704 & 3.517 & 0.123 & 3.237 & 3.123 & 0.112\\
    & \makebox[1.3cm][l]{$\text{\pamir}$}~\cite{zheng2020pamir} & \cmark & 2.035 & 1.873 & 0.079 & 1.936 & 1.263 & 0.078 & 2.216 & 1.611 & 0.093 & 2.122 & 1.495 & 0.088\\
    \hhline{~--------------}
    & $\text{\smplx GT}$ &  N/A & 1.518 & 1.985 & 0.072 & 1.335 & 1.259 & 0.085 & \textbf{1.070} & 1.058 & 0.068 & 1.158 & 1.125 & 0.074\\
    \hhline{~--------------}
    & $\text{\pifuSIM}$ &  \xmark & 2.688 & 2.573 & 0.097 & 2.100 & 2.093 & 0.091 & 2.973 & 2.940 & 0.111 & 2.682 & 2.658 & 0.104\\
    & $\text{\pamirSIM}$ & \cmark & 1.401 & 1.500 & 0.063 & 1.225 & 1.206 & \textbf{0.055} & 1.413 & 1.321 & 0.063 & 1.350 & 1.283 & \textbf{0.060}\\
    \hline
    \multirow{2}{*}{B} 
    & $\text{\modelname}_{\text{N}^{\dagger}}$ & \cmark & \textbf{1.153} & 1.545 & 0.057 & 1.240 & 1.226 & 0.069 & 1.114 & 1.097 & 0.062 & 1.156 & 1.140 & 0.064\\
    & \modelname w/o $\mathcal{F}_\text{n}^\text{b}$ & \cmark & 1.259 & 1.667 & 0.062 & 1.344 & 1.336 & 0.072 & 1.180 & 1.172 & 0.064 & 1.235 & 1.227 & 0.067 \\ 
    \hline
    \multirow{2}{*}{C} 
    & $\text{\modelname}_{\text{enc}(\mathcal{I},\predCloNormImgFB)}$ & \cmark  & 1.172 & \textbf{1.350} & \textbf{0.053} & 1.243 & 1.243 & 0.062 & 1.254 & 1.122 & 0.060 & 1.250 & 1.229 & 0.061 \\
    & $\text{\modelname}_{\text{enc}(\predCloNormImgFB)}$ & \cmark  & 1.180 & 1.450 & 0.055 & \textbf{1.202} & 1.196 & 0.061 & 1.180 & 1.067 & \textbf{0.059} & 1.187 & 1.110 & \textbf{0.060}\\
    \hline
    \multirow{4}{*}{D} 
    & $\text{\modelname}$ & \wcmark & 1.583 & 1.987 & 0.079 & 1.364 & 1.403 & 0.080 & 1.444 & 1.453 & 0.083 & 1.417 & 1.436 & 0.082\\
    & $\text{\modelname} + \text{BR}$ & \wcmark & 1.554 & 1.961 & 0.074 & 1.314 & 1.356 & 0.070 & 1.351 & 1.390 & 0.073 & 1.339 & 1.378 & 0.072\\
    & $\text{\pamirSIM}$ & \wcmark & 1.674 & 1.802 & 0.075 & 1.608 & 1.625 & 0.072 & 1.803 & 1.764 & 0.079 & 1.738 & 1.718 & 0.077\\
    \hhline{~--------------}
    & $\text{\smplx perturbed}$ & N/A & 1.984 & 2.471 & 0.098 & 1.488 & 1.531 & 0.095 & 1.493 & 1.534 & 0.098 & 1.491 & 1.533 & 0.097\\
    \hline
  \end{tabular}}
}
\vspace{-0.5 em}
\caption{
    Quantitative \change{evaluation} %errors
    (cm) for: 
    \textbf{(A)} performance \wrt SOTA; 
    \textbf{(B)} body-guided normal prediction; 
    \textbf{(C)} local-feature based implicit reconstruction; and 
    \textbf{(D)} robustness to \smplx noise. 
    Inference conditioned on: 
    (\cmark)    \smplx ground truth (GT); 
    (\wcmark)   perturbed \smplx GT; 
    (\xmark)    no \smplx condition. 
    \smplx ground truth is provided by each dataset. 
    \colorbox{Gray}{\cape} is not used for training, and tests generalizability.
}
\label{tab:benchmark}
\end{table*}



==> tabs/dataset.tex <==
\newcommand{\captionDATASETS}{
            Datasets for \threeD clothed humans. 
            Gray color indicates \colorbox{Gray}{datasets} used by \modelname. 
            The bottom ``number of scans'' row indicates the number of scans each method uses.
            The cell format is {\tt ~number\_of\_scans [method]}. 
            \modelname is denoted as {\tt [IC]}. 
            The symbol {\tt $\dagger$} corresponds to the ``8x'' setting in \cref{fig:datasize}.
}

\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|a|a|c|a|}
&\multicolumn{4}{c|}{Train \& Validation Sets}&\multicolumn{2}{c|}{Test Set}  \\  \hhline{~------}
& 
\rotatebox[origin=c]{0}{Renderp.}    & 
\rotatebox[origin=c]{0}{\twindom}    & 
\rotatebox[origin=c]{0}{\agora}      & 
\rotatebox[origin=c]{0}{\thuman}     & 
\rotatebox[origin=c]{0}{\buff}       & 
\rotatebox[origin=c]{0}{\cape}       \\ 
& 
\cite{renderpeople}         & 
\cite{twindom}              & 
\cite{patel2021agora}       & 
\cite{zheng2019deephuman}   & 
\cite{zhang2017buff}        &  
\cite{ma2020cape,ponsMoll2017clothCap}\\
\shline
Free \& public     &   \xmark   &   \xmark    &  \xmark    &   \cmark   &   \cmark    &    \cmark \\ 
Diverse poses      &   \xmark   &   \xmark    &  \xmark    &   \cmark   &   \xmark    &    \cmark \\ 
Diverse identities &   \cmark   &   \cmark    &  \cmark    &   \xmark   &   \xmark    &    \xmark \\ 
SMPL(-X) poses     &   \xmark   &   \xmark    &  \cmark    &   \cmark   &   \cmark    &    \cmark \\ 
High-res texture   &   \cmark   &   \cmark    &  \cmark    &   \xmark   &   \cmark    &    \cmark \\ 
\hline
\multirow{3}{*}{Number of scans} & \multicolumn{1}{l|}{450~\cite{saito2019pifu,saito2020pifuhd}} & 1000~\cite{zheng2020pamir} & ~~450~[IC] & ~~600~[$\text{IC}^{\dagger}$]  & ~~~~~5~\cite{saito2019pifu,saito2020pifuhd} & 150~[IC] \\
\qquad \quad  & \multicolumn{1}{l|}{375~\cite{huang2020arch}} & & ~3109~[$\text{IC}^{\dagger}$] & ~600~\cite{zheng2020pamir} & \multicolumn{1}{l|}{~~~26~\cite{huang2020arch}} & \\
& & & & & \multirow{1}{*}{~300~\cite{zheng2020pamir,li2020realtimeVolMoCap}} & \\
\end{tabular}
}
\vspace{-0.5 em}
\caption{\captionDATASETS}
\vspace{-0.3 em}
\label{tab:dataset}
\end{table}


==> tabs/perceptual_study.tex <==
\begin{table}
\centering
%\footnotesize
\small
\begin{tabular}{c|ccc}
 & \pifuSIM & \pifuhd~\cite{saito2020pifuhd} & \pamirSIM \\
\shline
Preference & 30.9\% & 22.3\% & 26.6\% \\
P-value & 1.35e-33 & 1.08e-48 & 3.60e-54 \\
\end{tabular}
\caption{
            Perceptual study. 
            Numbers denote the chance that participants prefer the reconstruction of a  competing method over \modelname for \inthewild images. 
            \modelname is judged significantly more realistic. 
}
\label{tab: perceptual study}
\end{table}


==> tabs/reb_ORIGINAL.tex <==
\begin{table}%[!htb]
\vspace{-0.2 em}
%
%
\hspace{-0.5 em}
\resizebox{0.5\linewidth}{!}{
\begin{minipage}{5.5cm}
\setlength{\parindent}{0em}
\addtolength{\tabcolsep}{-3pt}
\centering
\begin{tabular}{c|ccc}
    \multicolumn{1}{c|}{\# iters (460ms/it)} & 0 & 10 & 50\\
    \shline
    Chamfer $\downarrow$ & 1.417 & 1.413 & \textbf{1.339}\\
    P2S     $\downarrow$ & 1.436 & 1.515 & \textbf{1.378}\\
    Normal  $\downarrow$ & 0.082 & 0.077 & \textbf{0.074}\\
\end{tabular}
% \vspace{-1.0 em}
\caption{\modelname errors \wrt iterations}
\label{tab:loop}
\end{minipage}}
\hspace{-0.2 em}
\resizebox{0.5\linewidth}{!}{
\begin{minipage}{5.5cm}
\setlength{\parindent}{0em}
\addtolength{\tabcolsep}{-3pt}
\centering
\begin{tabular}{c|ccc}
    \multicolumn{1}{c|}{Receptive field} & 139 & 271 & 403\\
    \shline
    Chamfer $\downarrow$ & 1.418 & 1.478 & \textbf{1.366}\\
    P2S     $\downarrow$ & 1.236 & 1.320 & \textbf{1.214}\\
    Normal  $\downarrow$ & 0.083 & 0.084 & \textbf{0.078}\\
\end{tabular}
% \vspace{-1.0 em}
\caption{\pamir's receptive field}
\label{tab:rp}
\end{minipage}}
%
%
\vspace{-1.5 em} % plz let some breathing space (-2 is a bit too much)
%
%
\end{table}
%\vspace{-4mm}

